Relative algebraic K-theory by elementary means

In a previous paper I gave a presentation for the Quillen higher algebraic K-groups of an exact category in terms of "acyclic binary multicomplexes". In this paper I take that presentation as a definition of the higher K-groups, generalize it to the relative K-groups of an exact functor between exact categories, and produce the corresponding long exact sequence by elementary means, without homotopy theory.

==> Makefile <==
#-*- makefile-gmake -*-

NAME := rkgr

all : dvi ps.gz pdf dvi.gz
dvi : $(NAME).dvi
pdf : $(NAME).pdf
ps  : $(NAME).ps
ps.gz  : $(NAME).ps.gz
dvi.gz  : $(NAME).dvi.gz

# DVIPSFLAGS += -z
DVIPSFLAGS += -r
HEADERS = array.mps utils.mps sub.mps
INPUTS = mymacros.tex hamsplain.bst
TEX = latex
PDFTEX = pdflatex

.PHONY : all dvi pdf ps bak

# we include $(NAME).bbl for the sake of arxiv.org
TARFILES = Makefile $(NAME).tex $(INPUTS) papers.bib $(NAME).bbl mathpartir.sty

tar: $(NAME).tar.gz
$(NAME).tar.gz : $(TARFILES)
	tar cfz $@ $^
submission-tar: $(NAME)-s.tar.gz $(NAME).pdf  $(NAME).dvi
$(NAME)-s.tar.gz : $(TARFILES) $(NAME).pdf  $(NAME).dvi
	tar cfz $@ $^
	chmod a-w $@


test: $(NAME).tar.gz
	rm -rf tmpdir
	mkdir -p tmpdir
	cd tmpdir && tar xzf ../$(NAME).tar.gz && make

bak : $(NAME).tar.gz
	cvs ci -m ''
	scp -q $(NAME).tar.gz ssh.math.uiuc.edu:home/math/papers/me

%.epsu : %.eps $(HEADERS)
	cat $^ >$@

%.bux : %.tex
	$(TEX) '\scrollmode \input $<'
	rm -f $*.dvi
	cp $*.aux $*.bux
.PRECIOUS : %.bux %.ind
%.ind : %.idx
	makeindex $*.idx -o $*.ind.tmp
	! egrep '^(!! |   -- )' $*.ilg
	mv $*.ind.tmp $*.ind
%.bbl : %.bux
	cp $*.bux $*.aux
	bibtex $*
%.dvi : %.tex

once:
	$(PDFTEX) '\scrollmode \input $(NAME).tex'

%.dvi : %.bbl %.ind
	$(TEX) '\scrollmode \input $*'
	if grep -s "Rerun to get cross-references right." $*.log; \
	then $(TEX) '\scrollmode \input $*'; \
	fi
	! egrep "undefined on input line|There were undefined references" $*.log
%.pdf : %.bbl %.ind
	$(PDFTEX) '\scrollmode \input $*'
	if grep -s "Rerun to get cross-references right." $*.log; \
	then $(PDFTEX) '\scrollmode \input $*'; \
	fi
	! egrep "undefined on input line|There were undefined references" $*.log
%.ps : %.dvi
	dvips $(DVIPSFLAGS) $< $(OUTPUT_OPTION)
	rm -f body.tmp head.tmp
%.ps.gz: %.ps; gzip <$< >$@
%.dvi.gz: %.dvi; gzip <$< >$@
clean:; rm -f *.dvi *.numtex *.log *.xyc *.aux *.nums *.blg *.tmp *.bbl *.ps kbc.pdf *.bux kbc.tar.gz *.idx *.ilg *.ind *.out *.toc *.~*~ *.dvi.gz *.ps.gz
$(NAME).dvi $(NAME).idx $(NAME).bux : $(INPUTS)
$(NAME).bbl : papers.bib
print : $(NAME).ps
	lpr $<

upload:
	scp kbc.dvi kbc.dvi.gz kbc.ps.gz kbc.pdf u00:tmp

view : dc.dvi ; xdvi dc

shar : $(NAME).shar
$(NAME).shar : $(NAME).tex $(NAME).bbl
	shar $^ >$@

